Realizability Interpretation and Normalization of Typed Call-by-Need $$\lambda$$-calculus With Control

We define a variant of realizability where realizers are pairs of a term and a substitution. This variant allows us to prove the normalization of a simply-typed call-by-need $$\lambda$-$calculus with control due to Ariola et al. Indeed, in such call-by-need calculus, substitutions have to be delayed until knowing if an argument is really needed. In a second step, we extend the proof to a call-by-need $$\lambda$$-calculus equipped with a type system equivalent to classical second-order predicate logic, representing one step towards proving the normalization of the call-by-need classical second-order arithmetic introduced by the second author to provide a proof-as-program interpretation of the axiom of dependent choice.

==> figures/db_typing_rules.tex <==
\renewcommand{\hsep}{\qquad}
$$
\infer[\cboldrule]{\Gamma\vdash_v \cbold:A}{(\cbold:A )\in\S}
\hsep
\infer[\imprrule ]{\Gamma \vdash_v \lambda x_n.t:A \imp B }{\Gamma, x_n:A \vdash_t t:B & |\Gamma|=n}
\hsep
\infer[\xrule    ]{\Gamma \vdash_V x_n:A }{\Gamma(n)=(x_n:A)}
\hsep
\infer[\liftVrule]{\Gamma \vdash_V v:A }{\Gamma \vdash_v v:A }
$$
\vspace{\saut}
$$
\infer[\!\alphaboldrule]{\Gamma \vdash_F  \alphabold : A^\negt}{(\alphabold:A) \in\S}
~~\quad
\infer[\!\implrule     ]{\Gamma \vdash_F  t \cdot E:(A\imp B)^\negt}{\Gamma \vdash_t t:A ~&~ \Gamma \vdash_E  E:B^\negt}
~~\quad
\infer[\!\alpharule    ]{\Gamma \vdash_E \alpha_n:A^\negt}{\Gamma(n)=(\alpha_n:A^\negt)}
~~\quad
\infer[\!\liftErule    ]{\Gamma \vdash_E  F : A^\negt}{\Gamma \vdash_F  F : A^\negt}
$$
\vspace{\saut}
$$
\infer[\lifttrule]{\Gamma \vdash_t V:A }{\Gamma \vdash_V V:A }
\hsep
\infer[\murule   ]{\Gamma \vdash_t \mu\alpha_n.c:A}{\Gamma,\alpha_n:A^\negt \vdash_c c &  |\Gamma|=n}
\hsep
\infer[\lifterule]{\Gamma \vdash_e E:A^\negt}{\Gamma \vdash_E E:A^\negt}
\hsep
\infer[\mutrule  ]{\Gamma \vdash_e  \tmu x_n.c : A^\negt}{\Gamma, x_n:A \vdash_c c& |\Gamma|=n}
$$
\vspace{\saut}
$$
\infer[\eagerrule]{\Gamma \vdash_E  \tmu[x_i].\cut{x_i}{F}\tau : A^\negt}{\Gamma, x_i:A, \Gamma' \vdash_F F:A^\negt \quad \Gamma,x_i:A \vdash_\tau \tau:\Gamma'& |\Gamma|=i}
% \seq{\Gamma, x:A, \Gamma' \vdash_F F:A^\negt \quad \Gamma \vdash_\tau \tau:\Gamma'}
%     {\Gamma \vdash_E  \tmu[x].\cut{x}{F}\tau : A^\negt}
\hsep \hsep
\infer[\epsrule]{\Gamma \vdash_\tau \varepsilon:\varepsilon}{}
$$
\vspace{\saut}
$$
\infer[\tautrule]{\Gamma \vdash_\tau \tau[x_n:=t]:\Gamma',x_n:A}{\Gamma \vdash_\tau \tau:\Gamma' \hsep \Gamma,\Gamma' \vdash_t t:A & |\Gamma,\Gamma'|=n}
\hsep
\infer[\tauErule]{\Gamma \vdash_\tau \tau[\alpha_n:=E]:\Gamma',\alpha_n:A^\negt}{\Gamma \vdash_\tau \tau:\Gamma' \hsep \Gamma,\Gamma' \vdash_E E:A^\negt & |\Gamma,\Gamma'|=n}
% \seq{\Gamma \vdash_\tau \tau:\Gamma' \hsep \Gamma,\Gamma' \vdash_t t:A }
%     {\Gamma \vdash_\tau \tau[x:=t]:\Gamma',x:A}
%     \hsep
% \seq{\Gamma \vdash_\tau \tau:\Gamma' \hsep \Gamma,\Gamma' \vdash_E E:A^\negt }
%     {\Gamma \vdash_\tau \tau[\alpha:=E]:\Gamma',\alpha:A^\negt}    
$$
\vspace{\saut}
$$
\infer [\crule    ]{\Gamma \vdash_c \cut{t}{e} }{\Gamma \vdash_t  t:A & \Gamma  \vdash_e e:A^\negt}
\hsep\hsep
\infer[\lrule    ]{\Gamma \vdash_l c\tau}{\Gamma,\Gamma' \vdash_c c & \Gamma \vdash_\tau \tau : \Gamma'}
$$

==> figures/target_db_typing_rules.tex <==
$$
\infer[\axrule]{\Gamma;\Sigma \vdash x:A}{(x:A)\in\Gamma}
\qquad
\infer[\lamrule]{\Gamma;\Sigma \vdash \lambda x.t:A \imp B }
      {\Gamma,x:A ;\Sigma\vdash t:B & |\Gamma|=n}
\qquad
\infer[\apprule]{\Gamma;\Sigma\vdash t\,u: B }
      {\Gamma;\Sigma\vdash t:A\to B & \Gamma \vdash u:A}
$$
\vspace{\saut}
$$
\infer[\firule]{\Gamma;\Sigma\vdash \lambda\sigma.t : \forall X\subt\sto.A}
      {\Gamma;\Sigma,\sigma:X\subt\sto\vdash t:A & X \notin FV(\Gamma,\Sigma)}
\qquad
\infer[\ferule]{\Gamma;\Sigma\vdash t\,\sigma: A\{X:=\sto'\} }
      {\Gamma;\Sigma\vdash t:\forall X\subt\sto.A & \Sigma\vdash\sigma:\sto'\subt\sto}
$$
% $$
% \infer[\epsrule]{\Gamma;\Sigma \vdash \varepsilon:\ntrn{\tau}{\varepsilon}{\varepsilon}}{}
% \qquad
% \infer[\tautrule]{\Gamma;\Sigma \vdash [t]:\ntrn{\tau}{\sto_0}{A}}
%       {\Gamma;\Sigma\vdash t:\ntrn{t}{\sto_0}{A}}
% \qquad
% \infer[\tauErule]{\Gamma \vdash [t]:\ntrn{\tau}{\sto_0}A^\negt}
%       {\Gamma;\Sigma \vdash t:\ntrn{E}{\sto_0}{A}}
% $$
\vspace{\saut}
$$
\infer[\cboldrule]{\Gamma;\Sigma\vdash \cbold : A }{(\cbold:A)\in\S}
\qquad
\infer[\splitrule]{\Gamma;\Sigma\vdash \letin{x_{\tau_0},x,x_{\tau_1}}{\split\,\tau\,n}{t}:A}
      {\Gamma,x_{\tau_0}:\sto_0,x:A,x_{\tau_1}:\sto_1;\Sigma\vdash t:A & \Gamma\vdash \tau:\sto_0,B,\sto_1 & |\sto_0|=n}
$$
\vspace{\saut}
$$
\infer[\epsrule]{\Gamma;\Sigma\vdash \varepsilon:\ntrn{\tau}{\varepsilon}{\varepsilon}}{}
\qquad\qquad
\infer[\tautrule]{\Gamma;\Sigma\vdash [t]:\ntrn{\tau}{\sto}A}
      {\Gamma;\Sigma\vdash t:\ntrn{t}{\sto}{A} }
\qquad\qquad
\infer[\tauErule]{\Gamma;\Sigma\vdash [t]:\ntrn{\tau}{\sto}A^\negt}
      {\Gamma;\Sigma\vdash t:\ntrn{E}{\sto}{A} }
$$
\vspace{\saut}
$$
\infer[\taucatrule]{\Gamma \vdash \tau\tau':\ntrn{\tau}{\sto_0}\sto,\sto'}
      {\Gamma \vdash \tau:\ntrn{\tau}{\sto_0}\sto \qquad \Gamma\vdash \tau':\ntrn{\tau}{(\sto_0,\sto)}{\sto'}}
\qquad\qquad
\infer[\subtepsrule]{\Sigma\vdash\sigma:\sto'\subt \varepsilon }{}
$$
\vspace{\saut}
$$
\infer[\subtaxrule]{\Sigma\vdash\sigma:\sto'\subt \sto }{(\sigma:\sto'\subt\sto)\in\Sigma}
\qquad
\infer[\subturule]{\Sigma\vdash\sigma:(\sto',A)\subt(\sto,A)}{\Sigma\vdash\sigma:\sto'\subt\sto  & \sigma(|\sto|)=|\sto'| } 
\qquad
\infer[\subtdrule]{\Sigma\vdash\sigma:(\sto',A)\subt\sto    }{\Sigma\vdash\sigma:\sto'\subt\sto}
 $$
 


==> figures/target_typing_rules.tex <==
\setlength{\saut}{-0em}
$$
\infer[\crule]{\Gamma\vdash \cbold : X }{(\cbold:X)\in\S}
\qquad
\infer[\axrule]{\Gamma \vdash x:A }{(x:A)\in\Gamma}
\qquad
\infer[\lamrule]{\Gamma \vdash \lambda x.t:A \imp B }
      {\Gamma, x:A \vdash t:B}
\qquad
\infer[\apprule]{\Gamma \vdash t\,u: B }
      {\Gamma \vdash t:A\to B & \Gamma \vdash u:A}
$$
\vspace{\saut}
$$
\infer[\firule]{\Gamma \vdash t : \forall \compat{Y}{\sto}.A}
      {\Gamma,\compat{Y}{\sto}\vdash t:A & Y \notin FV(\Gamma)}
\qquad
\infer[\ferule]{\Gamma \vdash t: A\{Y:=\sto'\} }
      {\Gamma \vdash t:\forall \compat{Y}{\sto}.A & \Gamma\vdash\compat{\sto'}{\sto}}
% \qquad
% \infer{\Gamma \vdash t:B}
%       {\Gamma \vdash t:A & A\subt B}    
$$
\vspace{\saut}
$$
\infer[\splitrule]{\Gamma;\Sigma\vdash \letin{x_{\tau_0},x,x_{\tau_1}}{\split\,\tau\,y}{t}:B}
      {\Gamma,x_{\tau_0}:\sto_0,x:\ntrn{t}{\sto_0}{A},x_{\tau_1}:\ntrn{\tau}{(\sto_0,y:A)}{\sto_1}\vdash t:B & \Gamma\vdash \tau:\sto_0,y:A,\sto_1 }
$$
\vspace{\saut}
$$
\infer[\epsrule]{\Gamma \vdash \varepsilon:\ntrn{\tau}{\varepsilon}{\varepsilon}}{}
\qquad
\infer[\tautrule]{\Gamma \vdash [x:=t]:\ntrn{\tau}{\sto_0}{x:A}}
      {\Gamma\vdash t:\ntrn{t}{\sto_0}{A}}
\qquad
\infer[\tauErule]{\Gamma \vdash [x:=t]:\ntrn{\tau}{\sto_0}x:A^\negt}
      {\Gamma \vdash t:\ntrn{E}{\sto_0}{A}}
$$
\vspace{\saut}
$$
\infer[\taucatrule]{\Gamma \vdash \tau\tau':\ntrn{\tau}{\sto_0}\sto,\sto'}
      {\Gamma \vdash \tau:\ntrn{\tau}{\sto_0}\sto \qquad \Gamma\vdash \tau':\ntrn{\tau}{(\sto_0,\sto)}{\sto'}}
\qquad
\infer[\subtaxrule]{\Gamma\vdash \compat{\sto'}{\sto}}{(\compat{\sto'}{\sto})\in\Gamma}
\qquad 
\infer[\subtYrule]{\Gamma\vdash Y\subt Y}{}
$$
\vspace{\saut}
$$
\infer[\subtepsrule]{\Gamma\vdash \compat{\sto}{\varepsilon}}{}
\qquad
\infer[\subturule]{\Gamma\vdash \compat{(\sto',x:A)}{(\sto,x:A)}}{\Gamma\vdash\compat{\sto'}{\sto}}
\qquad
\infer[\subtdrule]{\Gamma\vdash \compat{\sto',\sto''}{\sto}}{\Gamma\vdash\compat{\sto'}{\sto}}
% \qquad
% \infer{\Gamma \vdash \tau:\ntrn{\tau}{\sto_0}{\sto}}
%       {\Gamma \vdash \tau:\ntrn{\tau}{\sto_0}{\sto'} & \Gamma\vdash\sto'\subt \sto}    
% \infer{\Gamma \vdash \tau:\sto}
%       {\Gamma \vdash \tau:\sto & \sto'\subt \sto}      
$$
\vspace{\saut}
$$
\infer[\subttransrule]{\Gamma\vdash\sto''\subt\sto}
    {\Gamma\vdash \sto''\subt\sto' & \Gamma\vdash\sto'\subt\sto}
\qquad
\infer[\tausubtrule]{\Gamma \vdash \tau:\ntrn{\tau}{\sto_0}{\sto}}
      {\Gamma \vdash \tau:\ntrn{\tau}{\sto'_0}{\sto'} 
	& 
	\Gamma\vdash\sto'\subt \sto
	&
	\Gamma\vdash\sto_0\subt \sto_0'}    
$$
\vspace{\saut}
% $$
% \infer{\Gamma \vdash A\subt A}{}
% \qquad~~
% \infer{\Gamma \vdash A \subt C}{\Gamma \vdash A\subt B & B\subt C}
% \qquad~~
% \infer{\Gamma \vdash A\to B \subt A' \to B'}{\Gamma \vdash A'\subt A & B\Gamma \vdash\subt B'}
% % \quad~~
% % \infer{\forall \compat{X}{\Gamma}. A \subt \forall \compat{X}{\Gamma'}.B}{A\subt B & \Gamma' \subt \Gamma}
% \qquad~~
% \infer{\Gamma \vdash\sto \subt \sto'}{\sto' \subseteq \sto}
% $$
\vspace{\saut}
$$
% \infer{(\union{\sto_0}{\sto'_0},\union{\sto_1}{\sto'_1})
% 	\subt \union{\sto_0,\sto_1}{\sto'_0,\sto'_1}}'}
% \qquad
\qquad
\infer[\subtsplitrule]{\Gamma\vdash t:B}{
      \Gamma[(Y_0,x:A,Y_1)/Y]\vdash t:B[(Y_0,x:A,Y_1)/Y]
      &
      \Gamma\vdash\compat{Y}{(\sto_0,x:A,\sto_1)}
      }
$$

